Measurement of azimuthal modulations in SIDIS off proton target at COMPASS

The azimuthal angle ($\phi_h$) distribution of hadrons produced in deep inelastic scattering serves as a powerful tool for probing the nucleon structure in terms of transverse momentum dependent parton distribution functions and fragmentation functions. For an unpolarized nucleon, three azimuthal modulations arise: $\cos\phi_h$ related to the Cahn effect, $\cos2\phi_h$ linked to the Boer--Mulders function, and $\sin\phi_h$ known as beam-spin asymmetry, each revealing insights into combinations of twist-two or higher-twist distribution and fragmentation functions. The COMPASS collaboration at CERN collected semi-inclusive deep inelastic scattering events in 2016 and 2017 using a longitudinally polarized 160 GeV/$c$ muon beam scattering off a liquid hydrogen target. Data from 2016 corresponding to about 1/3 of the full sample have been analyzed to measure the azimuthal modulations of charged hadrons. For the first time, the results were corrected for QED radiative effects using the DJANGOH MC generator.

==> bibliography.tex <==
%%% Bibliography (literature used as a source)
%%%
%%% We employ bibTeX to construct the bibliography. It processes
%%% citations in the text (e.g., the \cite{...} macro) and looks up
%%% relevant entries in the bibliography.bib file.
%%%
%%% The \bibliographystyle command selects, which style will be used
%%% for references from the text. The argument in curly brackets is
%%% the name of the corresponding style file (*.bst). Both styles
%%% mentioned in this template are included in LaTeX distributions.

% \bibliographystyle{plainnat}    %% Author (year)
 \bibliographystyle{unsrt}     %% [number]

\renewcommand{\bibname}{Bibliography}

%%% Generate the bibliography. Beware that if you cited no works,
%%% the empty list will be omitted completely.

\bibliography{bibliography}

%%% If case you prefer to write the bibliography manually (without bibTeX),
%%% you can use the following. Please follow the ISO 690 standard and
%%% citation conventions of your field of research.

% \begin{thebibliography}{99}
%
% \bibitem{lamport94}
%   {\sc Lamport,} Leslie.
%   \emph{\LaTeX: A Document Preparation System}.
%   2nd edition.
%   Massachusetts: Addison Wesley, 1994.
%   ISBN 0-201-52983-1.
%
% \end{thebibliography}

